Machine Learning Processes as Sources of Ambiguity: Insights from AI Art

Ongoing efforts to turn Machine Learning (ML) into a design material have encountered limited success. This paper examines the burgeoning area of AI art to understand how artists incorporate ML in their creative work. Drawing upon related HCI theories, we investigate how artists create ambiguity by analyzing nine AI artworks that use computer vision and image synthesis. Our analysis shows that, in addition to the established types of ambiguity, artists worked closely with the ML process (dataset curation, model training, and application) and developed various techniques to evoke the ambiguity of processes. Our finding indicates that the current conceptualization of ML as a design material needs to reframe the ML process as design elements, instead of technical details. Finally, this paper offers reflections on commonly held assumptions in HCI about ML uncertainty, dependability, and explainability, and advocates to supplement the artifact-centered design perspective of ML with a process-centered one.

==> analysis_table.tex <==
\begin{table}
 \caption{Overview of AI Art Examples Described in This Paper. (The numbers under ``Tactics'' refer to the list of tactics in section \ref{ambiguity_Lit})}
    \begin{tabular}{ | p{10em} | p{2em} | p{7em} | p{7em} | p{10em} | p{5em} | } 
      \hline
      Work  &   Year    &    Technology     &     Process Highlight  &   Types of Ambiguity  &   Tactics \\ 
      \hline
      \hline
      Biometric Mirror\cite{wouters_biometric_2019}     &   2018    &    Facial analysis   &   Application   &  Information, Context \& Relationship   &   2, 3, 4, 5, 8, 10   \\ 
      \hline
      Butcher's Son\cite{klingemann_butchers_2017}      &   2017    &   Image synthesis    &    Model training   &    Information    &   1, 3   \\ 
      \hline
      ImageNet Roulette\cite{paglen_imagenet_2019}      &   2019    &   Facial analysis   &    Data Curation \& Application  &    Information \& Relationship    &  2, 3, 4, 8, 10 \\ 
      \hline
      in\_transitu\cite{ada_ada_ada_in_transitu_2022}     &   2022    &   Facial analysis    &   Application     &    Information \& Relationship     &   2, 3, 4, 10 \\ 
      \hline
      Learning to See\cite{akten_learning_2019}      &    2017   &   Image synthesis    &   Application    &   Information \& Context     &   1, 2, 5  \\ 
      \hline
      Machine Bias\cite{yaszdani_machine_2018}      &   2018    &   Image synthesis   &   Data Curation    &   Information \& Relationship   &  1, 2, 4, 10 \\ 
      \hline
      Poison\cite{sivertsen_art_2023}      &   2021    &   Image synthesis    &    Model Training   &   Information \& Context   &   1, 3, 6, 7\\ 
      \hline
      POSTcard Landscapes from Lanzarote\cite{guljajeva_postcard_2022}      &   2020    &    Image synthesis   &   Data Curation    &   Information  &   1, 2 \\ 
      \hline
      Unsupervised\cite{anadol_unsupervised_2022}      &    2022   &    Image synthesis   &   Model Training    &    Information \& Context   &   1, 6, 7\\ 
      \hline
    \end{tabular}
    \label{table:1}
\end{table}

==> digital_art.tex <==
Glitch art is a type of art that is created by intentionally introducing errors or flaws into digital images or videos. These errors, known as "glitches," can be produced using various techniques, such as manipulating data or altering the hardware or software of a device. The resulting images or videos often have a distorted or abstract appearance that can be aesthetically interesting. 

Circuit bending is a similar technique that involves modifying the circuits of electronic devices, such as synthesizers or toys, to produce unusual or unpredictable sounds. This can be done by adding, removing, or rearranging circuits' components or applying external signals or voltages to the device. The resulting sounds are often strange or distorted and can be used in various musical or artistic contexts. Both glitch art and circuit bending involve manipulating technology in unexpected ways to create new and interesting forms of expression.

Specifically, in the context of glitch art and circuit bending, ambiguity may arise from the distorted or unexpected nature of the visual artefacts created by the glitches. As a result, the viewer may be uncertain about what they are seeing or interpret the glitches differently, adding a layer of ambiguity to the artwork's meaning.

The ambiguity concept is relevant to machine learning art and glitch art, but the way it manifests in each case may be slightly different. In the case of machine learning art, ambiguity may arise from the fact that the algorithms used to generate the art may produce unexpected or surprising results. The output of a machine learning algorithm can be challenging to predict or understand, and this can add an element of ambiguity to the resulting art.
In the case of glitch art, ambiguity may arise from the distorted or unexpected visual artefacts created by introducing errors or defects into digital images or video. These glitches can create a sense of uncertainty or confusion in the viewer, and they may interpret the glitches differently, adding a layer of ambiguity to the artwork.
Overall, the main difference between the two art forms is how ambiguity is generated. In machine learning art, it may arise from the unpredictable nature of the algorithms used to generate the art. In contrast, in the context of glitch art, it may arise from the visual distortions and artefacts created by the glitches.

In general, contemporary digital art movements refer to artistic practices that use digital technology as a medium or a means of creating art. New media art is a form of art that uses digital technology as a medium or a means of creating art. It is a contemporary art movement that emerged in the late 20th century and has continued to evolve and grow in the 21st century. New media art often incorporates interactivity, technology, and digital media elements into the artistic process and finished work. This can include various creative processes and forms of expression, such as video art, net art, digital painting, and generative art. New media art may also involve creative coding, virtual reality, or digital technology. Other types of new media art include:
Algorithmic art: This generative art is created using algorithms, which are sets of instructions that a computer can follow to produce a specific result. Examples are fractal geometry, cellular automata, and genetic algorithms.
Interactive art: This type of generative art involves creating a system or environment that responds to the actions or input of the viewer. Interactive art can be created using various technologies, such as sensors, cameras, or computer software, and can take many different forms, such as installations, games, or virtual reality experiences.
Data visualization: This generative art uses data to create visual representations or visualizations of information. This can be done using various techniques, such as graphs, charts, maps, or diagrams, and can be used to explore complex data sets, patterns, or relationships.
Machine learning art: This generative art uses machine learning algorithms to create art. Machine learning algorithms be used to create images, sounds, or other forms of art that are generated based on data or other input. For example, Style transfer: This technique allows an AI system to take an existing image and apply the style of another image to it. For example, an AI system could take a photo of a landscape and apply the style of a famous painting to it, creating a new and unique piece of art.
Evolutionary art: This AI art uses genetic algorithms to generate and evolve a population of images or other artistic creations over time. The AI system uses a set of rules or criteria to evaluate the artistic quality of each generation of images. Only the "best" images can survive and reproduce, resulting in a continually improving art population.
Net art, also known as internet art or online art, is a type of art created specifically for the internet or that uses the internet as a medium for its creation or display. It can include a wide range of media, from digital images and videos to websites and social media posts. Net art often explores the unique qualities of the internet as a medium, such as its global reach and ability to facilitate collaboration and communication.

some examples in chronological order and a link:

Artist: Frieder Nake
Artist: Kenneth C. Knowlton and Leon Harmon
Artist: Allan Kaprow
Artist: Nam June Paik
Artist: Maurizio Bolognini
Artist: Nam June Paik
Artist: Corey Arcangel
Artist: Petra Cortright
Artist: Trevor Paglen and Jacob Appelbaum

https://www.theartstory.org/movement/digital-art/


==> practice_review_draft.tex <==
% Suggestion: Should we add a review of some of the highlighted artworks from the NEURIPS workshop on Machine Learning for Creativity and Design? E.g. https://neuripscreativityworkshop.github.io/2021/#/gallery
% https://neuripscreativityworkshop.github.io/2022/
% https://www.aiartonline.com/category/art-2020/



\section{Review of Practice: Ambiguity in AI Art}

This section reviews work at the intersection of AI art and research. Drawing from our own practical work with creative uses of AI in art, design, and related contexts such as museum experiences, the authors collectively selected salient examples from works at the intersection of art and research. 

% We acknowledge that our personal bias may be introduced in the subjective selection criteria, and the number of works discussed here is relatively small. Our intention is not to make definitive claims about AI art but to offer a scoping study \cite{arksey2005scoping} to map key concepts and approaches in this relatively under-studied area of ambiguity in AI art.

One of the most well-known examples of artwork generated with a machine learning algorithm is a portrait titled {\em Edmond De Belamy} \cite{obvious_edmond_2018} (Fig. \ref{fig:training}, top right), which at first glance might look like any other contemporary painting. The portrait sits in a gold frame and shows a blurry image that vaguely resembles a human figure. However the artist's signature --- ``\(\min_{\mathcal{G}} \max_{\mathcal{D}} E_x \left[ log(\mathcal{D}(x)) \right] + E_Z \left[ log(1 - \mathcal{D}(\mathcal{G}(z))) \right] \)'' --- suggests that the painting was not created by a human. The signature, in fact, describes an algorithm which is part of the code in the DNN that generated these images, based on a training dataset of 15,000 portraits from the 14th to the 19th century. In 2018 {\em Edmond De Belamy} became the first AI art sold in Christie's, a well-established art auction house, for almost half a million dollars \cite{Vincent2018_Verge}. 

Some artworks similarly employ image generation algorithms to explore how this technology can be used to create new styles and types of images. For instance Hanny Töyryla describes the approach behind the artwork \textit{The House that is No Longer} as "using one neural model to reduce photos to contours, looking like woolen threads, and then to use this reduced image as a virtual printing plate, in another neural model, to produce a virtual art print eventually to be printed on fine art paper". According to the artist, this process often involves "a healthy dose of overfitting" in the training of the models in order to create a particular look \cite{toyryla_house_2018}. The resulting image is an ambiguous rendering of what seems to be parts of a sand-colored apartment building and black trees entangled in a chaotic composition. Another project, the MUNCH museum's installation \textit{Poison} \cite{munch_poison_2021} used \textit{underfitting} in order to recreate Edvard Munch's "green room" paintings in a way that reflected the ambiguity in the artist's various depictions of the same motif. This project aimed to investigate the use of technology-based immersive aesthetics as a form of art education. In the exhibition space, wall-sized interactive visuals generated by applying style transfer to 3D renderings based on original paintings by Edvard Munch were left intentionally unfinished. The project team decided to show underfitted results from earlier steps in the training process to evoke ambiguity.  

Upscaling, another highly technical method, has also been used. Generating high-resolution images is a computationally expensive process. Some models, such as Google's {\em Imagen} \cite{saharia2022photorealistic}, first generate low-resolution images (e.g., 64x64 pixels), and then employ a super-resolution model to scale the resulting image to a higher resolution (e.g., 1024x1024 pixels). %In the case of {\em Imagen}, the super-resolution model does not have access to the input text and hence might introduce details or artifacts unrelated to the human input to the system.
Mario Klingemann is an artist that uses this technique actively in his work. Using a technique called ``transhancement'' he upscales the images he creates using GAN. During this image-making process, artifacts are introduced that he embraces as part of the work. One of the artworks he has created using this technique is \textit{The Butcher's Son} \cite{klingemann_butchers_2017}.

In some artworks, the artists train models on specific and unusual types of data in order to explore the contrast between the training data and the artistic context, often with a critical perspective. An example of this is \textit{Learning to See} by Memo Akten \cite{akten_learning_2019} which appropriates GAN models trained on images of waves, flowers, and fire and applies them to real-time video feeds of phone chargers, pens, and fabric, resulting in varying compositions of either the waves, flowers, or fire that the models are trained on. However, applying these models to video feeds of everyday objects is kept ambiguous. The models keep generating pretty visuals and effectively disguise the bland everyday objects. 

Similarly, in \textit{POSTcard Landscapes from Lanzarote}, Varvara \& Mar collected public photographs from Flickr representing two perspectives on the island of Lanzarote \cite{guljajeva_postcard_2022}: landscape images and ``touristic'' images. These two categories are assumed to represent different visual perspectives. The resulting work consists of two videos, each showing morphing ambiguous imagery that at times vaguely resembles things like landscapes or airplanes, but most of the time escapes clear categorization (Fig. \ref{fig:curation}, bottom). Varvara \& Mar rely on the process and aesthetics of ML to open up a conversation about the tourist gaze vs. the local gaze. 

Some works take an even more overtly critical stance, using existing ML systems in art projects which expose problematic issues stemming from the underlying datasets and models used in these systems. An example which has received much attention is {\em ImageNet Roulette}\cite{paglen_imagenet_2019}, a digital app and AI art installation by Crawford \& Paglen (Fig. \ref{fig:curation}, middle). {\em ImageNet} \cite{imagenet} is one of the most widely used {\em training datasets} in machine learning \cite{Crawford2019_excavating}. The dataset contains 14 million labeled images organized into more than 20 thousand categories, and it has become a standard benchmark for computer vision research. {\em ImageNet Roulette} uses a NN that has been trained on a subset of {\em ImageNet} that is labeled under the ``person'' category. The app lets users upload their own photos to have them classified with categories in {\em ImageNet}'s ontology. {\em ImageNet Roulette} tends to return overly specific labels, often problematic if not outright offensive, such as "swot, grind, nerd, wonk, dweeb (...) rape suspect (...) first offender (...) gook, slant-eye" \cite{wong_viral_2019}. This problematic labelling seems to be a result of the way in which ImageNet has been constructed, using Mechanical Turk workers to label images corresponding to all the "synsets" in the lexical database WordNet. The artists explain their intention to call attention to how the {\em ImageNet} training dataset tries to resolve the ambiguity in images --- the ``potential meanings, irresolvable questions, and contradictions'' --- by compress[ing] and simplify[ing] images into deadpan banality'' \cite{Crawford2019_excavating}. By showing the audience how AI ``sees'' them as labels of {\em hyper specificity}, the artists let the audience directly confront the ``assumptions, politics, and worldviews'' often hidden in the enormous training datasets.

The system \textit{Biometric Mirror} created by Microsoft Research Centre for Social Natural User Interfaces \cite{wouters_biometric_2019} works in a similar fashion to explore the ethical implications of artificial intelligence and algorithmic decision-making. The system invites people to have their face photographed and analysed by a psychometric system, aiming to classify their faces on a range of dimensions from relatively overt traits such as age, gender and ethnicity to more diagnostic concepts such as aggressiveness, weirdness and emotional instability. The artwork \textit{in\_transitu} by Ada Ada Ada \cite{ada_ada_ada_in_transitu_2022} uses a similar approach to explore gender recognition by commercial image analysis systems. The artist, a trans woman, periodically uploads images of herself, naked from the waist up, along with the gender recognition output from five algorithms. While the photos show only small variation in hair style and facial expression the outputs from the algorithms vary widely, sometimes the same photo being classified by different algorithms as male and female with confidence levels near 100 \%. (All of the algorithms appear to treat gender as a binary variable that can be either male or female.)

In addition to working with existing datasets, critical artists may also create their own. Nushin Isabelle Yazdani, for her work \textit{Machine Bias} \cite{yaszdani_machine_2018}, created a dataset of around 3000 photographs of prison inmates from across the US. She trained a new DNN model to generate images of ``future faces of prisoners'', questioning predictive policing and automated pretrial risk assessment. Similar to {\em ImageNet Roulette}, this work exposes the pseudo-scientific assumptions of physiognomy, which believes that a person’s essential character can be observed through features of their bodies and faces, deeply entrenched in many face recognition applications. The central ambiguity of this work does not arise from the image labels in the dataset but rather from the epistemological foundation of all predictive technology --- past patterns in the dataset can predict the future. 

% These examples are representative of how they engage with the notion of ambiguity. What they have in common is how AI artists open the black box of DNNs to create a rich interpretative relationship between the audience and the AI. This type of work represents a considerable departure from the majority of current HCI design literature on ML products, which emphasizes the clarity and usability of the products (e.g., \cite{Amershi2019}) and frames uncertainty as a design challenge (e.g., \cite{yang_ml_hard}). While we acknowledge the importance of traditional HCI values, especially in real-world ML products, the rest of the paper attempts to provide alternative approaches by examining AI art through the lens of ambiguity. 


